Steadiface: Real-Time Face-Centric Stabilization on Mobile Phones

We present Steadiface, a new real-time face-centric video stabilization method that simultaneously removes hand shake and keeps subject's head stable. We use a CNN to estimate the face landmarks and use them to optimize a stabilized head center. We then formulate an optimization problem to find a virtual camera pose that locates the face to the stabilized head center while retains smooth rotation and translation transitions across frames. We test the proposed method on fieldtest videos and show it stabilizes both the head motion and background. It is robust to large head pose, occlusion, facial appearance variations, and different kinds of camera motions. We show our method advances the state of art in selfie video stabilization by comparing against alternative methods. The whole process runs very efficiently on a modern mobile phone (8.1 ms/frame).

==> implementation.tex <==
\subsection{Implementation Details}
\label{subsec:implementation}

We implement our algorithm with CPU/GPU co-processing
and test it on both the desktop and the Google Pixel 2,
which uses Qualcomm Snapdragon 835.
We implement OpenGLES shaders for the pyramid
creation and merge on GPU,
and implement alignment and noise estimation
on CPU using Halide \cite{Ragan-Kelley:2012:DAS}.
While the CPU-only implementation can still
achieve real-time throughput,
our joint CPU/GPU solution greatly reduces
the power consumption ($-66\%$).
We find that the existing spatial denoiser is effective enough for chroma channels,
and only enable our algorithm on the luma channel.
\vspace{-0.2in}
\input{noise_estimation}
